SimpliCity: Reconstructing Buildings with Simple Regularized 3D Models

Automatic methods for reconstructing buildings from airborne LiDAR point clouds focus on producing accurate 3D models in a fast and scalable manner, but they overlook the problem of delivering simple and regularized models to practitioners. As a result, output meshes often suffer from connectivity approximations around corners with either the presence of multiple vertices and tiny facets, or the necessity to break the planarity constraint on roof sections and facade components. We propose a 2D planimetric arrangement-based framework to address this problem. We first regularize, not the 3D planes as commonly done in the literature, but a 2D polyhedral partition constructed from the planes. Second, we extrude this partition to 3D by an optimization process that guarantees the planarity of the roof sections as well as the preservation of the vertical discontinuities and horizontal rooftop edges. We show the benefits of our approach against existing methods by producing simpler 3D models while offering a similar fidelity and efficiency.

==> presentation/tallinn_full.tex <==
\begin{table*}[t]
    \captionsetup{font=LARGE,singlelinecheck=off}
    % \captionsetup{singlelinecheck=off}

    \setlength{\tabcolsep}{9pt}
\centering
\caption[]{\textbf{Quantitative evaluation.}
\begin{itemize}
    \item $|V|$ is the number of vertices of the models
    \item $|F|$ is the number of triangles of the models
    \item $\recall$ is the distance from the input point cloud to the models
    \item $\precision$ is the distance from the reconstructed to reference model
    \item Time is average runtime per building. 
  \end{itemize}
  For each metric and each dataset, we highlight the \colorbox{blue!25}{best} and \colorbox{blue!10}{second best} average scores. $^\dagger$We stop the process after a runtime of 5 min per building.
% \TODO{Probably best to simplify this table, and put this one as an appendix. E.g. mean values of all cities and mean of the two Chamfer distances would make it more readable and would probably make us best or second best on most metrics.}
}
\vspace{-0.2cm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l|lrrrrrrrrrr@{}}
\toprule
\multicolumn{2}{c}{}                            &\multicolumn{3}{c}{\emph{Complexity}}& \multicolumn{2}{c}{\emph{Accuracy}}   & \multicolumn{4}{c}{\emph{Failure}}     & \emph{Perform.} \\
\midrule
\multicolumn{2}{c}{}                            & $|V|$         & $|F|$         &$E_{<0.5~\text{m}}$&  $\recall$    &  $\precision$         &  HO             & VO          & SI  &  Total & Time     \\
\multicolumn{2}{c}{}                            &               &               &  [\%]             & [cm]          &               [cm]    &                   &          &    &         &     [s] \\
\midrule
% Tallinn
\multirow{4}{*}{\rotatebox[origin=c]{90}{\hspace{-6mm}\emph{Tallinn (3471)}}}
&\textbf{2.5DC}~\cite{zhou2010dualcontouring}       &    112        & 187           & \tf 2.86 &  11.9     & 81.9      &     -     &   -    & -   & 0           & \tf 0.13  \\
&\textbf{KSR}                                       & \ts 67.8      & \ts 71.4      &    8.35  & \ts 8.07  &      15.9 &     -     &   -    & -   & 3           & 10.4      \\
&\textbf{Geoflow}~\cite{peters2022geoflow}          &    180        & 172           &    28.0  & \tf 7.18  & 36.4      &     -     &   -    & -   & 0           & \ts 4.03  \\
&\textbf{City3D}$^\dagger$~\cite{huang2022city3d}   &    116        & 199           &    25.0  & 9.39      & \tf  7.24 &     -     &   -    & -   & 291         & 49.1      \\
% &\textbf{OursComplex}                               &     39.1      &     72.6      &   7.63   & 7.74      & \ts  12.4 &     -     &   -    & -   & 0           & \ts 1.59  \\
% &\textbf{OursNoReg}                                 & \tf 33.6      & \ts 61.1      &   7.63   & 7.74      & \ts  12.4 &     -     &   -    & -   & 0           & \ts 1.59  \\
&\textbf{Ours}                                      & \tf 32.2      & \tf 58.2      & \ts 4.39 &     9.34  &  \ts 13.2 &     45    &  810   & 40  & 895 (26\%)  & 4.19      \\
\midrule
% % Zurich min_inliers = 50
% \multirow{4}{*}{\rotatebox[origin=c]{90}{\hspace{-7mm}\emph{Zurich50}}}
% &\textbf{2.5DC}~\cite{zhou2010dualcontouring}       & 140           & 241           & \bf23.7   & 57.2      &           & 4     & \bf 0.052 \\
% &\textbf{KSR}~\cite{bauchet2020kinetic}             &  79.8         & \bf 99.2      &    38.6   &     37.6  &           & 17    & 6.52 \\
% &\textbf{KSR+}~\cite{bauchet2020kinetic}            &  79.8         & \bf 99.2      &    38.6   &     37.6  &           & 17    & 6.52 \\
% &\textbf{Geoflow}~\cite{peters2022geoflow}          &  194          & 188           &   38.8    & 57.3      &           & 108   & 1.59\\
% &\textbf{City3D}$^\dagger$~\cite{huang2022city3d}   & 107           & 184           &   41.7    & \bf29.7   &           & 259   & 42.3 \\
% &\textbf{Ours}                                      & \bf 57.4      & 109           &    39     &      33   & 0.21      &\bf 0  & 1.09 \\
% % &\textbf{OursReg} & \bf 31.5         & \bf 56.3        &     15.4 &     42.0 & \bf 0.95 && 3.19 \\
% \midrule
% Zurich min_inliers = 20
\multirow{4}{*}{\rotatebox[origin=c]{90}{\hspace{-6mm}\emph{Zurich (3195)}}}
&\textbf{2.5DC}~\cite{zhou2010dualcontouring}       & 140           & 241           &  \tf 2.57 & \tf 16.4  & 50.6      &    -      &  -    &   -   &    6        & \tf 0.052 \\
&\textbf{KSR}~\cite{bauchet2020kinetic}             &  116          & \ts  139      &   8.72    & \ts 22.0  &     33.2  &    -      &  -    &   -   &    22       & 6.52 \\
&\textbf{Geoflow}~\cite{peters2022geoflow}          & 227           & 220           &   27.0    &   28.1    & 50.0      &    -      & -     &   -   &    97       &  \ts 1.59\\
&\textbf{City3D}$^\dagger$~\cite{huang2022city3d}   & \ts 112       & 193           &   28.3    &   30.6	& \tf 20.0  &    -      & -     &   -   &    501      & 42.3 \\
% &\textbf{OursNoReg}                                 & \ts 66.6      & \ts  126      &     16.3  &    24.2   &      25.6 & -         &  -    &   14  &   14        & \ts 1.09 \\
&\textbf{Ours}                                      & \tf 58.3      & \tf  109      &  \ts 7.48 &    26.6   & \ts 26.0  &  929      & 141   & 103   & 1073 (33\%) & 3.82 \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\hspace{0mm}\emph{Helsinki (1180)}}}
&\textbf{2.5DC}~\cite{zhou2010dualcontouring}       & \ts      570  &      1045     &  \tf 2.67 & \tf 22.6  & 69.9      &  -        &   -   &  -    & 3           & \tf 1.15 \\
&\textbf{KSR}~\cite{bauchet2020kinetic}             &     619       & \ts   704     &   14.5    &    39.8   & \ts 39.2  &  -        &   -   &  -    & 0           & 67.9 \\
&\textbf{Geoflow}~\cite{peters2022geoflow}          & 900           & 883           &   23.1    &     34.2  & 54.7      &  -        & -     &  -    &   63        & \ts 6.12\\
% &\textbf{OursNoReg}                                 & \tf 230       & \ts  423      &   12.2    &    37.2   & \tf 27.6  & -         &  -    &  1    &   1         &    \ts 1.09 \\
&\textbf{Ours}                                      & \tf  214      &  \tf  393     &  \ts 9.5  &\ts 32.3   &  \tf 37.1 & 459       &    32 &  281  & 772 (65\%)  & 6.81 \\
\bottomrule
\end{tabular}
}
\label{tab:tallinn}
\end{table*}

==> presentation/tallinn_ours_only.tex <==
\begin{table*}[t]
    \captionsetup{font=LARGE,singlelinecheck=off}
    % \captionsetup{singlelinecheck=off}

    \setlength{\tabcolsep}{9pt}
\centering
\caption[]{\textbf{Quantitative evaluation.}
\begin{itemize}
    \item $|V|$ is the number of vertices of the models
    \item $|F|$ is the number of triangles of the models
    \item $\recall$ is the distance from the input point cloud to the models
    \item $\precision$ is the distance from the reconstructed to reference model
    \item HO signifies an error in the horizontal optimisation
    \item VO signifies an error in the vertical optimisation
    \item Total = HO+VO    
    \item WT is the percentage of buiding meshes which are watertight 
    \item IF is the percentage of buiding meshes which are intersection-free 
  \end{itemize}
For each metric and each dataset, we highlight the \colorbox{blue!25}{best} and \colorbox{blue!10}{second best} average scores.
% \TODO{Probably best to simplify this table, and put this one as an appendix. E.g. mean values of all cities and mean of the two Chamfer distances would make it more readable and would probably make us best or second best on most metrics.}
}
\vspace{-0.2cm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l|lrrrrrrrHrrrr@{}}
\toprule
\multicolumn{2}{c}{}                            &\multicolumn{3}{c}{\emph{Complexity}}& \multicolumn{2}{c}{\emph{Accuracy}}   & \multicolumn{6}{c}{\emph{Error}}     & \emph{Perform.} \\
\midrule
\multicolumn{2}{c}{}                            & $|V|$         & $|F|$         &$E_{<0.5~\text{m}}$&  $\recall$    &  $\precision$         &  HO          & VO     & SI    &  Total    &   WT  & IF    & Time     \\
\multicolumn{2}{c}{}                            &               &               &  [\%]             & [cm]          &               [cm]    &              &        &       &           &       &       &  [s] \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\hspace{-6mm}\emph{Tallinn (3471)}}}
&\textbf{OursComplex}                           &     39.1      &     72.6      &   7.63            & 7.74          & \tf  12.4             &     -         &   -    & -   & 0          & 0.58  & 0.40  & \tf 1.59  \\
&\textbf{OursNoReg}                             & \ts 33.6      & \ts 61.1      &   7.63            & 7.74          & \tf  12.4             &     -         &   -    & -   & 0          & 0.58  & 0.40  & \tf 1.59  \\
&\textbf{Ours}                                  & \tf 32.2      & \tf 58.2      & \ts 4.39          &     9.34      &  \ts 13.2             &     45        &  810   & 40  & 855 (26\%) &  0.59 & 0.37  &\ts 4.19      \\
\end{tabular}
}
\label{tab:tallinn}
\end{table*}
